ZeroReg: Zero-Shot Point Cloud Registration with Foundation Models

State-of-the-art 3D point cloud registration methods rely on labeled 3D datasets for training, which limits their practical applications in real-world scenarios and often hinders generalization to unseen scenes. Leveraging the zero-shot capabilities of foundation models offers a promising solution to these challenges. In this paper, we introduce ZeroReg, a zero-shot registration approach that utilizes 2D foundation models to predict 3D correspondences. Specifically, ZeroReg adopts an object-to-point matching strategy, starting with object localization and semantic feature extraction from multi-view images using foundation models. In the object matching stage, semantic features help identify correspondences between objects across views. However, relying solely on semantic features can lead to ambiguity, especially in scenes with multiple instances of the same category. To address this, we construct scene graphs to capture spatial relationships among objects and apply a graph matching algorithm to these graphs to accurately identify matched objects. Finally, computing fine-grained point-level correspondences within matched object regions using algorithms like SuperGlue and LoFTR achieves robust point cloud registration. Evaluations on benchmarks such as 3DMatch, 3DLoMatch, and ScanNet demonstrate ZeroReg's competitive performance, highlighting its potential to advance point-cloud registration by integrating semantic features from foundation models.

==> sec/tables/tab_3dmatch_other.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.0} % 减少行距，使表格更紧凑
\centering
\tabcolsep 3pt % 减少列间距
\caption{Registration Recall (RR) and Inlier Ratio (IR) on 3DMatch and 3DLoMatch for Transferred and Ours. 
The \textbf{highest} performance is shown in bold.}
\resizebox{\columnwidth}{!}{%
\label{exp:tab:3d_3dl_2}
\begin{tabular}{>{\columncolor{gray!50}}l >{\columncolor{gray!50}}c >{\columncolor{gray!50}}c >{\columncolor{gray!50}}c >{\columncolor{gray!50}}c >{\columncolor{gray!50}}c}
    \toprule[1pt]
    \rowcolor[HTML]{FFFFFF} 
    \multirow{2}{*}{\textbf{Method}} & \vspace{2pt}\multirow{2}{*}{\shortstack{\textbf{Train on} \\ \textbf{ 3DMatch}}} & \multicolumn{2}{c}{\textbf{3DMatch}} & \multicolumn{2}{c}{\textbf{3DLoMatch}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
    \rowcolor[HTML]{FFFFFF} & & \textbf{RR (\%)} & \textbf{IR (\%)} & \textbf{RR (\%)} & \textbf{IR (\%)} \\ 
    \midrule[0.8pt]
    \rowcolor[HTML]{FFFFFF} \multicolumn{6}{l}{\textbf{Transferred zero shot way}} \\
    \cdashline{1-6}[2pt/2pt]
    FreeReg~\cite{wang2023freereg} & $\times$ & 41.2 & - & 15.1 & - \\ 
    Ours & $\times$ & 86.2 & - & 52.1 & - \\
    \bottomrule[1pt]
\end{tabular}%
}
\end{table}

==> sec/tables/tab_different_method.tex <==
\begin{table}[t]
\centering
\caption{Comparison of different configurations of ZeroReg on 3DMatch and 3DLoMatch datasets. The table shows the impact of object-level (detection, segmentation) and point-level (SuperGlue or LoFTR) components on registration recall (RR) and inlier ratio (IR).}
\label{tab:zeroreg_comparison}
\setlength{\tabcolsep}{4pt} % Adjust column spacing
\renewcommand{\arraystretch}{1.1} % Adjust row spacing
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Configuration}} & \multicolumn{2}{c}{\textbf{Object-Level}} & \multicolumn{2}{c}{\textbf{Point-Level}} & \multicolumn{2}{c}{\textbf{3DMatch}} & \multicolumn{2}{c}{\textbf{3DLoMatch}} \\
& \textbf{Detection} & \textbf{Segmentation} & \textbf{SuperGlue} & \textbf{LoFTR} & \textbf{RR(\%)} & \textbf{IR(\%)} & \textbf{RR(\%)} & \textbf{IR(\%)} \\
\midrule
\textbf{ZeroReg (Full Model)} & \checkmark & \checkmark & \checkmark & - & \textbf{92.5} & \textbf{74.3} & \textbf{81.4} & \textbf{55.8} \\
\cdashline{1-9}[2pt/1pt]
\rowcolor{gray!20} ZeroReg (w/o Detection) & - & \checkmark & \checkmark & - & 89.1 & 70.2 & 78.3 & 51.7 \\
ZeroReg (w/o Segmentation) & \checkmark & - & \checkmark & - & 88.0 & 68.5 & 77.0 & 50.5 \\
\rowcolor{gray!20} ZeroReg (w/ LoFTR) & \checkmark & \checkmark & - & \checkmark & 91.2 & 72.8 & 80.1 & 54.2 \\
ZeroReg (w/o Detection, w/ LoFTR) & - & \checkmark & - & \checkmark & 87.5 & 67.9 & 76.0 & 49.3 \\
\midrule
\textbf{Baseline Comparison} & \multicolumn{4}{c|}{SuperGlue Only} & 85.4 & 66.2 & 74.3 & 47.1 \\
\rowcolor{gray!20} & \multicolumn{4}{c|}{LoFTR Only} & 86.5 & 67.8 & 75.5 & 48.5 \\
\bottomrule
\end{tabular}%
}
\end{table}
